Receiver Placement for Speech Enhancement using Sound Propagation Optimization

A common problem in acoustic design is the placement of speakers or receivers for public address systems, telecommunications, and home smart speakers or digital personal assistants. We present a novel algorithm to automatically place a speaker or receiver in a room to improve the intelligibility of spoken phrases in a design. Our technique uses a sound propagation optimization formulation to maximize the Speech Transmission Index (STI) by computing an optimal location of the sound receiver. We use an efficient and accurate hybrid sound propagation technique on complex 3D models to compute the Room Impulse Responses (RIR) and evaluate their impact on the STI. The overall algorithm computes a globally optimal position of the receiver that reduces the effects of reverberation and noise over many source positions. We evaluate our algorithm on various indoor 3D models, all showing significant improvement in STI, based on accurate sound propagation.

==> reviews.tex <==
1. Introduction: CAD design for speech. Speech has become important and with devices Alexa. What are the implications for CAD?

Use similar introduction as Noise

2. Previous Work: Include more on propagation, optimization; 


4. Section 4: We need a lot more details on STI is integrated with optimization and the modified Simulated Annealing. Need more Math details.

What are the challenges and issues with handling speech-related optimization.




Importance/Relevance: Of sufficient interest
Comment on Importance/Relevance:
Interesting topic also from 6DoF audio point of view.

Novelty/Originality: Moderately original

Technical Correctness: Probably correct
Comment on Technical Correctness:
Technical contribution is relatively small, but the problem description and solution description is interesting.

Experimental Validation: Limited but convincing
Comment on Experimental Validation:
The validation part is somewhat lacking. It is not clear whether real recording positions were tested, or were the simulated signals evaluated. Overall results part is quite unclear.

Clarity of Presentation: Difficult to read
Comment on Clarity of Presentation:
Some parts are quite vague what have been done. Results part is particularly unclear.

-----tance/Relevance: Irrelevant or out of scope
Comment on Importance/Relevance:
The authors refer to a relevant final application context, which is automatic speech recognition at distance from microphones, under noisy and reverberant conditions. This is a quite relevant scientific topic. However, I do not think that the contents of this paper may be interesting for most researchers in the field, due to reasons explained below.
Impor

Novelty/Originality: Minor originality
Comment on Novelty/Originality:
There may be some originality in the approach proposed in this work. I would suggest the authors to study the effectiveness of their approach in a more solid and realistic experimental ASR framework.

Technical Correctness: Has major problems
Comment on Technical Correctness:
I do not find this work technically correct for many reasons explained elsewhere. Here, I would just add that a realistic simulation of impulse response, between source and receiver, plays a fundamental role in a work as this one. The use of the technique proposed in the end of section 3.2, rather than alternative ones, is not justified. I would also suggest the authors to use real impulse responses, and to measure them, in order to better support their research.

Experimental Validation: Insufficient validation
Comment on Experimental Validation:
Experimental results are just reported in terms of STI improvement. I would have expected to see an activity also involving the adoption of an automatic speech recognition task, possibly based on real-world speech signals, since in such context simulations may produce a misleading experimental evidence.

Clarity of Presentation: Difficult to read
Comment on Clarity of Presentation:
I find this work rather weak in terms of focus. The title itself is misleading: why “noise reduction”, if the goal is to select from a set of possible receiver locations? The experimental setup should be better described, for instance to show the reliability of simulated speech data that were used in the experiments.

Reference to Prior Work: Does not cite relevant work
Comment on Reference to Prior Work:
The literature is full of works on distant speech recognition and on automatic microphone selection, which are not mentioned by the authors, and are quite relevant as reference for their work. See also the works related to international challenges, such as REVERB, CHiME, ACE, etc., organized during the past 5-10 years

General Comments to Authors:
The paper proposes an algorithm to compute an optimal placement of the microphone based on STI, which aims to minimize the impact of indoor environmental noise and reverberation. Based on the title, and on what reported in the introduction, I understood that the main goal of the work was to show advantages of the proposed solution when applied in the context of automatic speech recognition. However, the work reports only results concerning intelligibility improvements.
From my point of view, the contribution of the paper is rather limited, also in terms of novelty of the proposed solution. I would suggest the authors to expand their work with speech recognition experiments based on multi-microphone setting and on the use of real noisy speech signals, in order to verify the advantages of their algorithms.


-----

General Comments to Authors:
The authors propose to compute the optimal receiver position to maximize the speech intelligibility as measured by transmission index (STI) in complex configurations of the enclosure, speech source, noise source and the receiver. In that sense the proposed approach is complementary to speech denoising approaches, wherein the receiver position is fixed and the goal is to process the received signal to increase the SNR or intelligibility etc. The paper is fairly well written and easy to comprehend. My main concerns regarding this paper are with respect to the practicality of such an algorithm and insufficient validation of the proposed idea as detailed below:
1. The authors assume that the source is loud enough for the receiver to be placed anywhere to maximize the STI as governed by the RIR. This is seldom true in practice.
2. In the results section the authors show that the proposed algorithm predicts the optimal receiver position to be away from the noise source and a reflective floor. These results are quite intuitive for any sound engineer. So, with all the computationally tedious process of computing RIR of each and every location on a grid of possible source locations and computing the STI at each of those locations, it is not clear what we gain that is not already obvious. So, the authors must include some cases where a sound engineer’s intuition would not be as good as the algorithm’s recommendation for the receiver’s position.
3. How can this be done in practice? This would require RIR estimation at several points within the enclosure, the need for which must be justified more thoroughly int he paper.
4. Although the STI is a measure of speech intelligibility, it may be worthwhile to conduct a perception test to judge how significant this improvement is.
In addition to these major concerns, there are a few minor concerns as listed below:
1. The “Suburban” scene layout is not shown.
2. Throughout the paper there is a confusing terminology pertaining to automatic speech
recognition and speech recognition by human subjects. This should be resolved by referring to speech recognition by human subjects as just speech intelligibility (perhaps?). Because STI in an indicator for speech intelligibility and not a metric for ASR. For instance the first sentence in Sec 3.3 - “ In a typical environment where speech recognition is used, having a high STI for a single source location is not sufficiently optimal for the entire environment.”
4. It would be good to add a reference for Sabine’s equation, in Section 4.


